A Deep Learning Approach To Estimation Using Measurements Received Over a Network

We propose a novel deep neural network (DNN) based approximation architecture to learn estimates of measurements. We detail an algorithm that enables training of the DNN. The DNN estimator only uses measurements, if and when they are received over a communication network. The measurements are communicated over a network as packets, at a rate unknown to the estimator. Packets may suffer drops and need retransmission. They may suffer waiting delays as they traverse a network path. Works on estimation often assume knowledge of the dynamic model of the measured system, which may not be available in practice. The DNN estimator doesn't assume knowledge of the dynamic system model or the communication network. It doesn't require a history of measurements, often used by other works. The DNN estimator results in significantly smaller average estimation error than the commonly used Time-varying Kalman Filter and the Unscented Kalman Filter, in simulations of linear and nonlinear dynamic systems. The DNN need not be trained separately for different communications network settings. It is robust to errors in estimation of network delays that occur due to imperfect time synchronization between the measurement source and the estimator. Last but not the least, our simulations shed light on the rate of updates that result in low estimation error.

==> RW-age-estimation.tex <==
\subsection{Age of Information and State Estimation}
\label{age-estimation}
There is a growing importance for the  availability of timely and updated information in cyber-physical systems where sources transmit their (periodic or sporadic) fresh status to a destination (insert reference). Consider a cyber-physical system, where a number of sensors are sampled and transmit the corresponding  freshness-sensitive data (e.g., temperature, humidity, location of an autonomous vehicle) to a destination over a wireless channel. Under ideal conditions, this destination receives fresh data continuously. Although, in reality, due to the imperfect and lossy channel, a status update from the source might have aged because of the queuing and transmission delay. In such cases, it is vital for the system to jointly design the sensors sampling policy at the source and estimation strategy at the remote destination. Authors in~\cite{huang-2019, huang-2020}, and~\cite{fountoulakis-2020} have designed sensor sampling policy along with a communication protocol between sensor and controller indicating that, re-transmissions of packets might not always be useful, as outdated data can in-turn hurt remote estimation. Although, their designed optimal policy is conditioned on the network channel conditions and a small number of packet drops, which also bound the mean squared error (MSE) metric (probability of packet dropouts that system can handle is not clearly defined).

==> RW-contribution.tex <==
\subsection{Contribution}
\begin{itemize}
    \item we already know  Optimal Kalman estimator for intermittent and aged observations with an infinite buffer .
    \item Do we know optimal controller for such a system of intermittent and aged observations? We have stable controller but not the optimal, control design is independent of estimator design (separation principle holds when controller has knowledge of what control input plant has used)
    \item Any model on control also delivered to controller in a packet- not yet, say any agent wants to know what control input is used by other agents in the environment, thus saying that control inputs are also delayed over the edge network. Kalman is only optimal under the condition that it knows the control used.
    \item Under model free settings, for partially observable environments, MARL community talk about communication under limited bandwidth constraints, although whenever any agent is scheduled to broadcast their messages, they broadcast the latest observation at their end instead of an aged observation. Hence, the information of one particular agent is aged only in respect with when the agent was scheduled and not in respect to its own observation. The next aspect is memory based learning, where availability of memory is necessary to learn any particular tasks, say to pick an action in Atari games, agent has to memorise the frames. Another task includes any agent learning to estimate position and velocity from sensor observations as explained in \cite{meng-2021}, but how much loss of observation can the agent handle in order to predict, any observation is either reset to 0 or removed completely with some probability, still not talks about highly aged observations and how it can impact the estimator.
\end{itemize}

==> RW-control-design.tex <==
\subsection{Controller Design}
 The authors in~\cite{tipsuwan-2003, hespanha-2007, zhang-2015, park-2017}, and~\cite{zhang-2019} summaries control design to ensure system stability for NCSs in events of network induced delays and packet dropouts. The control designs are widely segregated into time-triggered, event triggered and self-triggered control laws. For time-triggered control laws, the gains are designed by considering delays which can be smaller/larger than a sampling period. These control gains can either be constant real matrix (for small delays) or a function of input delays (for large delays).  The optimal controller under such conditions assumes prior knowledge of delay along with full state information. Though such an assumption is conservative, the optimal gains are designed to ensure bounded state error covariance. Authors further provide a threshold value for maximum packet dropouts, beyond which system stability is unbounded. In order to maximise control performance across heterogeneous control loops, authors in \cite{ayan-2021} propose a scheduling policy, since each sensor in a control loop maintains an infinite FCFS packet queue. Their proposed constant control gain can be obtained by solving the discrete time algebraic Ricatti equation, independent of network(packet dropouts/input delays)(investigate the difference).
 
 Though in many practical scenarios, complexity of network dynamics can pose harder problem to determine the network evolution model in advance. Model-free learning enables the decision-making agents to adapt their behavior based on interaction with the environment and build an understanding of underlying system model evolution. Authors in~\cite{jaehyun-2017} aims to learn a pattern of network-induced effects on maneuvers of UAVs, given the difficulty of modeling such autonomous systems. To simplify their model, they initialize their system matrices to identity matrices and learn state estimates given bounded input delays and packet dropouts. The work in~\cite{kiumarsi-2018} reviews reinforcement  learning based feedback control solutions for optimal regulation and tracking of single and multi-agent systems.


==> RWlearning.tex <==
%bib file age-learning
\label{learning-network}
\subsection{Learning system parameters in  MDPs and POMDPs}
Data driven model-free learning techniques have been applied to optimize age-of-information for different network assumptions and applications in~\cite{ceran-elif-2019, ceran-elif-2018, beytur-hasan-2019, elgabli-anis-2019}, and~\cite{leng-shiyang-2019age}. The underlying goal is to learn policies that schedule updates from one or more sources to minimize age the destination. Authors in~\cite{ceran-elif-2019} and~\cite{yin-bo-2020} aim to schedule updates of a source over an error prone channel under different feedback mechanisms including ARQ and Hybrid ARQ.


However sensor observations don't always entirely represent the state of the environment. Due to complex and unknown  underlying system evolution model, only a few works study the Partially Observable Markov Decision Process (POMDPs). Partial observability can arise from different sources which includes the importance of remembering past and temporarily available information like maneuvers of autonomous vehicles in navigation tasks, sensor limitations or noise, unobserved variations of plant under applied control, road occlusions and blind spots on roads \cite{hubmann-2018-Transaction}, \cite{hubmann-2018-ITSC}. Resolution of partial observability can either be solved by maintaining a belief state, given the received observations so far or build model-free approaches that learn to build memories based on interaction with the environment \cite{heess-2015}. The former approach requires the need for a model added with the computational cost of maintaining the belief state. The latter approach uses the feature representation of observations and build associations among them, ran over many steps.  Works~\cite{abedin-sarder-2020, abd-mohamed-2019} learn trajectories of one or more Unmanned Aerial Vehicles (UAVs) that collect information from sensors such that average AoI is minimised to a threshold at the ground station.   However, one would also like to choose trajectories such that energy efficiency is maximized. In~\cite{yi-mengjie-2020} and~\cite{abd-mohamed-2019}, deep reinforcement learning is used to find the trajectory for the UAV under its energy constraints with the aim of minimising AoI at the UAV and ground nodes.

Traditionally, state estimation and path planning are solved using Kalman Filters(KFs). KF gives optimal estimates and control, given system equations are linear and typically noise (process and measurement) are uncorrelated and white Gaussian. Neural networks are widely used for state representation and control problems. Recurrent neural networks(RNN) allow feedback connections between neurons, thus forming dynamical systems. RNNs are able to store information for a longer duration (memory) and are also robust towards any noise in the input. A number of previous works have analysed how stored memory can help learn policies for different control tasks. Designing efficient controller requires perceiving the entire underlying state at a decision point which is not feasible for real time tasks given noisy and incomplete state information. The work in~\cite{hausknecht-2015} devised control policy on Atari 2600 games by adding LSTM in order to extract memory of partially observable game frames. Similarly, in~\cite{zhu-2017} Action-specific Deep Recurrent Q-network (ADRQN) is used by including history of action spaces along with history of observations on discrete action spaces. Though~\cite{heess-2015} and~\cite{zhang-2016} studied the efficacy of adding LSTM to deep learning algorithm by extending on continuous control tasks with partial observations. DIAL~\cite{foerster-2016} learns what to communicate by back-propagating all the other agents’ gradients to the
message generation network.  SchedNet~\cite{kim-2019} learns a weight-based scheduler to determine the communication priority based on DIAL. Although all such tasks don't account for network constraints and the packet losses due to network imperfections. The work in~\cite{meng-2021} investigates the importance of recent observations  as a part of the input to RNNs in order for the agent to learn appropriate control policy. Despite their control tasks, their algorithm fails if agent receives no recent observation for long duration of time. How much history is necessary for such a task and how much observation loss, it can suffer still remains unanswered. Finally, the work in~\cite{mao-2020}- learning under limited bandwidth and message pruning.

==> estimates_kalman_lstm.tex <==
\section{State Estimation}
\subsection{Dynamic Process Modelling} 

Consider a linear time invariant (LTI) plant $\mathcal{P}$, whose state evolution is governed by,
	\begin{align}
		\mathcal{P}:x_{k+1}  & =A x_{k}+B u_k^a +w_k,\\
		Y_{k} &= C x_{k}+v_{k},
	\end{align}
	where, $x_{k} \in \mathbb{R}^n$ represents the state of plant $\mathcal{P}$, at a discrete time instant  $k\in\{0,1,2\dots\}$, $A \in \mathbb{R}^{n \times n}, B \in \mathbb{R}^ {n \times p}$ and $C \in \mathbb{R}^{m \times n}$ denotes the state transition, control and observation matrix respectively. The control input used by the plant is denotes by $u_k^a \in \mathbb{R}^{p}$ and $Y_{k} \in \mathbb{R}^{m}$ represents the measurement vector generated by the sensor. $w_{k}$ and $v_{k}$ are the process and measurement noise sampled from an independent and identically distributed zero mean Gaussian processes, with covariance matrices $Q_k$ and $R_k$ respectively. We assume	covariance matrix of process and measurement noise are time invariant, $Q_k = Q$ and $R_k = R$.
	
	The sensors measure the states of the plant remotely and send such measurements to could server, where the measurements are transmitted back to the plant, representing an infrastructure. The described setup of a  \emph{networked closed-loop system} is illustrated in Figure~\ref{fig:architecture}, where a camera system captures the states of the plant and transmits to a cloud server followed by a transmission back to the plant. The remote sensor and plant can be represented by a source-destination communication pair. Let $G_s(k)$ represent the most \emph{recent} measurement received at the plant (destination). Due to the presence of a queuing system, $G_s(k)$ is a random variable. The \emph{Age of Information} (AoI) of the state (source, $s$) at the plant (destination) for a time instant $k$ is defined,
	\begin{equation}
	    \label{eq:AoI_def}
	    \Delta_{s,k} = k - G_s(k).
	\end{equation}
	Let $\gamma_k \in \{0,1\}$ represent a random time varying binary quantity indicating whether a measurement (packet) is received at the plant. In a discrete time system the AoI evolution is governed by,
	\begin{equation}
	    \begin{cases}
	        \Delta_{s,k} = \Delta_{s,k} + 1, & \text{if } \gamma_k = 0, \\
	        \Delta_{s,k} = k - G_s(k), & \text{otherwise},
	    \end{cases}
	\end{equation}
	with the assumption $\Delta_{s,0} = 1$.
	It is shown in \cite{nelson-2013} that LTI state-feedback estimator suffices to achieve optimal performance under state-feedback information, although  in the absence of a delayed network, thus, motivating the need to develop an estimator with stale state information.   
	
	\begin{align}
		\mathcal{I}_{\mathcal{P},k} &= \{Y_k ,u_k^a, \Delta_{u,k}\}\\
		\mathcal{I}_{c,k} &= \{(\hat{Y}_{k})_{\mathcal{P}}, \Delta_{s,k}, \hat{\Delta}_{u,k}\} 
	\end{align}
	At time $k$, a packet generated by the plant $\mathcal{P}$ contains $[k, \Delta_{u,k}, Y_k]$, \textit{i.e}, the packet  generation timestamp, plant's used control input and its measurements. Plant can also generate separate packets for its used control input as $[k,\Delta_{u,k}]$ in addition to a packet with its measurement vector ($Y_k$).
	$\mathbf{\Delta_{s,k}} \triangleq k - G_s(k)$ is the age of measurement at the controller, where $G_s(k)$ is the timestamp of the freshest measurement at the controller. 
    $\mathbf{\Delta_{u,k}}\triangleq k - G_u(k)$ is the age of control input at the plant, where $G_u(k)$ is the time stamp of the freshest control packet at the plant. $\widehat{Y}_k = Y_{k-\Delta_{s,k}}$ is the freshest measurement at the controller. $u_k^a=u_{k-\Delta_{u,k}}^c$ is the control input used by the plant at $k$. $\mathbf{\hat{\Delta}_{u,k}}\triangleq k - \widehat{G_u}(k)$ is the estimate of age of the control input used by the plant, at the controller, where $\widehat{G_u}(k)$ is the time stamp of the freshest control input of the plant at the controller.
    $\{(.)_{\mathcal{P}}\}$ denotes the packet information from the plant available on the controller at $k$.
	
	
	
	 At time step $k$, controller maintains the estimate of control input $\hat{u}_{k}^a$ used by the plant. Controller estimates the plant states as,
     
         %\begin{subequations}
    	 %\begin{align*}
    	%	\hat{x}_{k}^- &= A\hat{x}_{k-1}^+ + B \hat{u}_{k-1}^a\\
    	%	\hat{u}_{k-1}^a &= u_{(k-1)-\hat{\Delta}_{u,{k-1}}}^c\\
    	%	\hat{x}_{k}^+ &=
    	%	\begin{cases}
    	%		\begin{matrix}
    	%		A^{\Delta_{s,k}}\hat{x}_{k-\Delta_{s,k}}^- + & \text{} \\ K(Y_{k-\Delta_{s,{k}}}-C \hat{x}_{k-\Delta_{s,{k}}}^-) + & \text{, Packet received} \\
    	%		\sum\limits_{i=1}^{\hat{\Delta}_{u,k}}A^{i-1}B u^c_{k-\hat{\Delta}_{u,k}} & \text{on Controller}
    	%		\end{matrix}  \\ %A^{\Delta_{s,k}}\hat{x}_{k-\Delta_{s,k}}^-+K(Y_{k-\Delta_{s,{k}}}-C \hat{x}_{k-\Delta_{s,{k}}}^-) +\vspace{0.1in}\\
    			%\hspace{50pt}\sum\limits_{i=1}^{\hat{\Delta}_{u,k}}A^{i-1}B u^c_{k-\hat{\Delta}_{u,k}} &\quad\text{Packet received on Controller}\\
    	%		\hat{x}_{k}^-, \quad\quad  \text{otherwise}
    	%	\end{cases}
    	%\end{align*}
	    %\end{subequations}
     
	\begin{align*}
		\hat{x}_{k}^- &= A\hat{x}_{k-1}^+ + B \hat{u}_{k-1}^a\\
		\hat{u}_{k-1}^a &= u_{(k-1)-\hat{\Delta}_{u,{k-1}}}^c\\
	\end{align*}
	\begin{align*}
	    	\hat{x}_{k}^+ & =
		\begin{cases}
		    \begin{matrix}
		        A^{\Delta_{s,k}}\hat{x}_{k-\Delta_{s,k}}^- + \\ 
		        K(Y_{k-\Delta_{s,{k}}}-C \hat{x}_{k-\Delta_{s,{k}}}^-) + \\ \sum\limits_{i=1}^{\hat{\Delta}_{u,k}}A^{i-1}B u^c_{k-\hat{\Delta}_{u,k}}
		    \end{matrix}, & \text{if } \gamma_k = 1\\ 
			\hat{x}_{k}^-, & \text{otherwise}
		\end{cases}
	\end{align*}
	
	


==> literature_long_draft.tex <==
\section{Literature}


\subsection{State Estimation in NCSs}
Real-time remote estimation is critical for networked control
applications such as industrial automation, smart grid, vehicle
platooning, drone swarming, autonomous transportation systems and intelligent manufacturing systems. An estimator in a network control loop predicts states by using the intermittent measurements of the system \cite{hespanha-2007}. %These predicted states are in turn used for determining control inputs as the estimator compensates for any measurement(sensor) noise, network delays and packet losses \cite{park-2017}. 
These predicted states are in turn used for determining control inputs. Furthermore, the estimator compensates for any measurement(sensor) noise, network delays and packet losses \cite{park-2017}. Kalman filter is a widely used state estimator for a range of NCS applications~\cite{sinopoli-2004}, \cite{schenato-2008}, \cite{schenato-2007},  \cite{lu-2021} and \cite{moayedi-2011}. The works in~\cite{sinopoli-2004, schenato-2008, schenato-2007, minyong-2017, liang-2017, rosenthal-2017, lee-2018, lu-2021} study states estimators performance for intermittent, delayed or periodic packets at controller and/or delayed control input at the actuator. However the dynamic system stability and bounds for estimation error covariance is determined only for a small set or range of acceptable critical packet success probability in~\cite{sinopoli-2004, schenato-2008, schenato-2007, minyong-2017} or under a mapping of Eigenvalue of state transition matrix with packet drop probability \cite{liang-2017}. 

Optimal control design with estimation is studied in~\cite{schenato-2007, liang-2017}, and~\cite{rosenthal-2017}. The authors show that an optimal estimator and controller can be designed independently (separation principle) based on the protocol supporting acknowledgement (delayed as well as instantaneous) of transmitted packet/control input. However, this separation principle doesn't hold for UDP-like protocol since estimator error covariance depends on the control input (input reference). Furthermore, the work in~\cite{lee-2018} designed optimal controller assuming the knowledge of a constant delay. Similarly, in~\cite{lu-2021}, the authors use Smith-predictor to derive the optimal controller to compensate for a bounded (check) input delay.

A consolidated study covering models for network control systems ranging from small and large network delays, packet dropout models in sensor-controller channel, estimation with intermittent and delayed measurements and optimal control are presented in~\cite{tipsuwan-2003, hespanha-2007, srinivasan-2014, zhang-2015, park-2017}, and~\cite{zhang-2019}.
\newline
\input{age-estimation}
\input{learning}
\input{control-design}
\input{contribution}


==> results.tex <==
\section{Evaluation}
\label{sec:evaluation}
% \begin{figure}[htbp]
% \begin{minipage}[t]{0.5\linewidth}
%     \includegraphics[width=\linewidth]{ICC-2021/Results/Baseline_Linear_Age_0.3.pdf}
%     \caption{\small Comparison of LSTM-AA and the TVKF when controls are known.}
%     \label{fig:baselinear_age}
% \end{minipage}%
%     \hfill\hfill%
% \begin{minipage}[t]{0.5\linewidth}
%     \includegraphics[width=\linewidth]{ICC-2021/Results/Baseline_nonlinear_age0.3.pdf}
%     \caption{\small Comparison of LSTM-AA and the UKF when controls are known.}
%     \label{fig:baseline_nonlinear_age}
% \end{minipage} 
% \end{figure}


% \begin{figure}[t]
% \begin{center}
% \subfloat[]{\includegraphics[width = 0.5\linewidth] {Results/Baseline_Linear_Age_0.3.pdf}
% \label{fig:baselinear_age}}
% \subfloat[]{\includegraphics[width = 0.5\linewidth] {Results/Baseline_nonlinear_age0.3.pdf}
% \label{fig:baseline_nonlinear_age}}
% \caption{\small Comparison of LSTM-AA and (a) the TVKF and (b) the UKF, for when controls are known.}
% \label{fig:baseline_comparisons}
% \end{center}
% \vspace{-0.2in}
% \end{figure}

\begin{figure}[t]
\begin{center}
\subfloat[]{\includegraphics[width = 0.5\linewidth] {Results/Baseline_Linear_Age_0.3_barplot.pdf}
\label{fig:baselinear_age}}
\subfloat[]{\includegraphics[width = 0.5\linewidth] {Results/Baseline_nonlinear_age0.3_barplot.pdf}
\label{fig:baseline_nonlinear_age}}
\caption{\small Comparison of LAA and (a) the TVKF and (b) the UKF, for the \emph{known controls} setting.}
\label{fig:baseline_comparisons}
\end{center}
\vspace{-0.2in}
\end{figure}

% \begin{figure*}[h]
% 	\begin{center}
% 		\subfloat[]{\includegraphics[width = 0.25\linewidth]{ICC-2021/Results/agevsnoage_0.3_linear.pdf}
% 			\label{fig:agevsnoage_0.3_linear}}
% 		\subfloat[]{\includegraphics[width = 0.25\linewidth]{ICC-2021/Results/agevsnoage_0.5_linear.pdf}
% 			\label{fig:agevsnoage_0.5_linear}}
% 		\subfloat[]{\includegraphics[width = 0.25\linewidth]{ICC-2021/Results/agevsnoage_0.3_nonlinear.pdf}
% 			\label{fig:agevsnoage_0.3_nonlinear}}
% 		\subfloat[]{\includegraphics[width = 0.25\linewidth]{ICC-2021/Results/agevsnoage_0.5_nonlinear.pdf}
% 			\label{fig:agevsnoage_0.5_nonlinear}}
% 		\caption{Do we need age? (a) Unknown Control, Linear q =$0.3$. (b) Unknown Control, Linear q =$0.5$. (c) Unknown Control, Non Linear q =$0.3$. (d) Unknown Control, Non Linear q =$0.5$.}	
% 	\end{center}
% 	\label{fig:AgeOrNot}
% 	\vspace{-0.3in}
% \end{figure*}



% \begin{figure*}[h]
% 	\begin{center}
% 		\subfloat[]{\includegraphics[width = 0.25\linewidth]{ICC-2021/Results/noisy_linear_0.3.pdf}
% 			\label{fig:noisy_linear_0.3}}
% 		\subfloat[]{\includegraphics[width = 0.25\linewidth]{ICC-2021/Results/noisy_linear_0.5.pdf}
% 			\label{fig:noisy_linear_0.5}}
% 		\subfloat[]{\includegraphics[width = 0.25\linewidth]{ICC-2021/Results/noisy_nonlinear_0.3.pdf}
% 			\label{fig:noisy_nonlinear_0.3}}
% 		\subfloat[]{\includegraphics[width = 0.25\linewidth]{ICC-2021/Results/noisy_nonlinear_0.5.pdf}
% 			\label{fig:noisy_nonlinear_0.5}}
% 		\caption{Impact of noisy age estimates (a) Unknown Control, Linear q =$0.3$. (b) Unknown Control, Linear q =$0.5$. (c) Unknown Control, Non Linear q =$0.3$. (d) Unknown Control, Non Linear q =$0.5$.}	
% 	\end{center}
% 	\label{fig:L_1_game}
% 	\vspace{-0.3in}
% \end{figure*}
We used the learning algorithm, described in Algorithm~\ref{alg:learning-LAA} to train a LAA model for each of the following network and dynamic system settings. For both the linear system and the cartpole, we trained a model for each $(p,q)$ in the list $(0.01, 0.3)$, $(0.1, 0.3)$, $(0.297, 0.3)$, $(0.01, 0.5)$, $(0.3, 0.5)$, $(0.499, 0.5)$. We also trained a model, wherein each episode of training we randomly chose $q$ in $(10^{-2}, 1)$ and $p$ in $(10^{-3}, q)$\footnote{We sample uniformly from the range of $log10$ probabilities to ensure a good representation of probabilities $<< 1$.}. Note that it is essential for queue stability to choose $p < q$. We will refer to the former settings as \emph{fixed network} and the latter as \emph{time-varying network}.

Further, for each fixed-network setting, we perform an ablation study to answer whether the age $\age_{\vvec{y}}(t)$ at the input of LAA (see Equation~(\ref{eqn:input_LSTM})) makes a significant difference to the estimation error. To do so, we train a LAA model, for each fixed network setting, without age as an input. We will refer to this as the \emph{No Age} setting.

Last but not the least, for each fixed-network setting, we train a LAA model, for when the current values of $u_{x,k}, u_{y_k}$ and $F_k$ are assumed to be known to the estimator, respectively for the linear system and the cartpole. These models help us baseline the performance of LAA, as we explain later. The acceleration values $u_{x,k}, u_{y_k}$ serve as control actions for the linear system. Similarly the force $F$ serves as a control action for the cartpole. This when the control actions are assumed known is referred to as the \emph{known control} setting.

In this section, we test the trained models that take age as an input for when the true age is available and also when a noisy estimate of the same is available. We also test the fixed network models that don't take age as input. The performance metric of interest is the estimation error, which is the square-root of the average squared measurement residual defined in Section~\ref{sec:approxArch}. We show a comparison of the estimation error achieved by the LAA models, for the linear dynamic system, with the commonly used Time-Varying Kalman Filter (TVKF), and for the cartpole, with the Unscented Kalman Filter (UKF). The average error is computed over $200$ episodes, wherein each episode is $40000$ time steps long.
% Say something about testing...
% SA: We test the trained models on both linear and nonlinear dynamic systems for $M=200$ episodes with each episode $T =40000$ time slots long. The range of measurement vectors for both the systems and the communication network remains same as that described in~\ref{ref:simulated_env} and~\ref{sec:communication_networks}. Although we also choose to train LAA over a range of choices of $p$ and $q$ which we describe in next section.
%We describe the empirical takeaways obtained from training and testing our proposed architecture on our simulated worlds. We quantify the estimation performance of LAA and the baseline algorithms using \emph{Estimation Error}, which is the square-root of the average squared measurement residual defined in Section~\ref{sec:approxArch}.

\textbf{Baselining LAA using the known control setting:} 
We begin by showing a comparison of LAA for the \emph{known control} setting. For this setting, the baseline algorithms of Time-Varying Kalman Filter (TVKF) and the Unscented Kalman Filter (UKF) for the non-linear dynamic system are expected to do well. Both TVKF and the UKF assume knowledge of the dynamic system model. 

The TVKF with infinite time buffer for linear dynamic system is in fact known to be the optimal estimator~\cite{schenato-2008-optimal} when the current controls used by the target are always known to the estimator. This gives us an opportunity to benchmark the data-driven LAA against a known optimal estimator. We compare the estimation error obtained using the LAA models trained for the \emph{known control} setting with that obtained using the TVKF for the linear system. Figure~\ref{fig:baselinear_age} compares the estimation error obtained using LAA and the TVKF for the linear dynamic system. The algorithms are compared for when $q=0.3$ and $p$ takes values of $0.01$ (low rate and high age, see Figure~\ref{fig:averageAgevsp}), $0.1$ (close to the age optimal rate), and $0.297$ (high rate, delay, and age). \emph{As is seen from the figure, LAA performs almost as well as the optimal TVKF.}

For a nonlinear dynamic system, we were only able to find a UKF implementation~\cite{li-2012-stochastic} that works with intermittent updates. However, an update when received is assumed current (fresh, age $0$). We modify the UKF implementation in the following manner. When an update is not received, we propagate the prior state estimates and error covariance according to the system dynamic model and set the posterior of the state and error covariance to their respective priors. When a new update arrives, we use it to recalculate the posterior estimates corresponding to the timestamp of the update, and propagate the estimates up to the current time using the model. Figure~\ref{fig:baseline_nonlinear_age}, compares LAA and UKF. \emph{LAA compares well with UKF.}
% \begin{figure}[h]
% 	\begin{center}
% 		\subfloat[]{\includegraphics[trim = 0cm 0cm 0cm 1cm, width = 0.5\linewidth, clip]{Results/agevsnoage_0.3_linear.pdf}
% 			\label{fig:agevsnoage_0.3_linear}}
% 		\subfloat[]{\includegraphics[width = 0.5\linewidth]{Results/agevsnoage_0.3_nonlinear.pdf}
% 			\label{fig:agevsnoage_0.3_nonlinear}}
% 		\caption{\small Controls are communicated over the network for $q=0.3$. (a) Linear system,  (b) Nonlinear. Results for $q=0.5$ are not shown but look similar.}
% 		\label{fig:AgeOrNot}
% 	\end{center}
% 	\vspace{-0.3in}
% \end{figure}

\begin{figure}[t]
\begin{center}
\subfloat[]{\includegraphics[width = 0.5\linewidth] {Results/agevsnoage_0.3_linear_barplot.pdf}
\label{fig:agevsnoage_0.3_linear}}
\subfloat[]{\includegraphics[width = 0.5\linewidth] {Results/agevsnoage_0.3_nonlinear_barplot.pdf}
\label{fig:agevsnoage_0.3_nonlinear}}
\caption{\small Controls are communicated over the network for $q=0.3$. (a) Linear system,  (b) Nonlinear. Results for $q=0.5$ are not shown but look similar.}
\label{fig:AgeOrNot}
\end{center}
\vspace{-0.2in}
\end{figure}


\textbf{LAA's performance for the fixed network setting, with and without age inputs:}
As in typically the case, the control actions, unlike for baselining, are obtained over the network. We assume that the TVKF and the UKF use the last known control till a more recent packet containing controls is received over the network. For the linear system, Figure~\ref{fig:agevsnoage_0.3_linear} compares the estimation error obtained by LAA (\emph{fixed network} setting), LAA with \emph{No Age}, and the TVKF. Figure~\ref{fig:agevsnoage_0.3_nonlinear} does the same for the cartpole with the UKF chosen instead of the TVKF. It is clear that LAA with the age inputs does the best and in fact outperforms the TVKF and the UKF. LAA without the age inputs performs fairly well when $p$ is set close to the age optimal rate but suffers otherwise. \emph{Keeping the age inputs $\vvec{\age_u}$ and $\vvec{\age_y}$ clearly benefits estimation. Also, see Figures~\ref{fig:baseline_comparisons} and~\ref{fig:AgeOrNot}, all estimators give a much smaller estimation error when the chosen $p$ is the age optimal rate.}

%Figure~\ref{fig:AgeOrNot} compares LAA trained with and without the age inputs $\vvec{\age_u}$ and $\vvec{\age_y}$. Figure~\ref{fig:agevsnoage_0.3_linear} is for the linear dynamic system and also shows the performance of the TVKF. Figure~\ref{fig:agevsnoage_0.3_nonlinear} is for the nonlinear system and shows the performance of the UKF. LAA for both when age is input and not was trained and tested for $300$ episodes for each $p,q$. 

\textbf{LAA's performance when age estimates are noisy:} In practice, getting an accurate estimate of age requires the source of the measurement and the estimator to be time-synchronized. This is often imperfect and typically not available. A typoical workaround is to estimate one-way delays using round-trip-time (RTT) (between source and estimator) measurements. The one-way delay estimates can then be used to estimate age, which recall is the time elapsed between generation of a measurement and its reception at the estimator.

For the purpose of evaluating the impact of noisy age estimates on LAA's performance, we scale the true age by a continuous uniform random variable that takes values in $(0,2)$, where a scaling of $2$ approximates a RTT based estimate of age. To the scaled value we add a Gaussian with mean $0$ and standard deviation equal to $10\%$ of the true age. Figure~\ref{fig:noisyAgeEst} shows the impact of noisy age estimates on the estimation error. Note that LAA was trained as earlier with true age values at its input. Noisy age estimates were only provided when testing. \emph{The estimation performance of LAA is not very impacted, unlike the TVKF and the UKF that see a significant increase in estimation error in comparison to when the true age is available.}
 
% \begin{figure}[t]
% 	\begin{center}
% 		\subfloat[]{\includegraphics[width = 0.5\linewidth]{Results/noisy_linear_0.3.pdf}
% 			\label{fig:noisy_linear_0.3}}
% % 		\subfloat[]{\includegraphics[width = 0.25\linewidth]{ICC-2021/Results/noisy_linear_0.5.pdf}
% % 			\label{fig:noisy_linear_0.5}}
% 		\subfloat[]{\includegraphics[width = 0.5\linewidth]{Results/noisy_nonlinear_wukf_0.3.pdf}
% 			\label{fig:noisy_nonlinear_0.3}}
% % 		\subfloat[]{\includegraphics[width = 0.25\linewidth]{ICC-2021/Results/noisy_nonlinear_0.5.pdf}
% % 			\label{fig:noisy_nonlinear_0.5}}
% 		\caption{\small Impact of noisy age estimates (a) Linear $q=0.3$ (b) Nonlinear $q=0.3$. Controls are communicated over the network.}	
%     	\label{fig:noisyAgeEst}		
% 	\end{center}
% 	\vspace{-0.2in}
% \end{figure}

\begin{figure}[t]
	\begin{center}
		\subfloat[]{\includegraphics[width = 0.5\linewidth]{Results/noisy_linear_0.3_barplot.pdf}
			\label{fig:noisy_linear_0.3}}
% 		\subfloat[]{\includegraphics[width = 0.25\linewidth]{ICC-2021/Results/noisy_linear_0.5.pdf}
% 			\label{fig:noisy_linear_0.5}}
		\subfloat[]{\includegraphics[width = 0.5\linewidth]{Results/noisy_nonlinear_wukf_0.3_barplot.pdf}
			\label{fig:noisy_nonlinear_0.3}}
% 		\subfloat[]{\includegraphics[width = 0.25\linewidth]{ICC-2021/Results/noisy_nonlinear_0.5.pdf}
% 			\label{fig:noisy_nonlinear_0.5}}
		\caption{\small Impact of noisy age estimates (a) Linear $q=0.3$ (b) Nonlinear $q=0.3$. Controls are communicated over the network.}	
    	\label{fig:noisyAgeEst}		
	\end{center}
	\vspace{-0.2in}
\end{figure}

\textbf{Does LAA train well over a time-varying network setting? Or do we need to train it separately for every fixed network setting of interest?} To have to train LAA separately for fixed network settings would make it impractical. Often, the network parameters aren't known and change over time. Figures~\ref{fig:TimeVaryingNtwkTrain} and~\ref{fig:TimeVaryingNtwkTrain_0.007} compare the testing performance of LAA trained over a time-varying network with the testing performance of LAA trained for the same fixed network parameters that are used for testing. \emph{Figures~\ref{fig:generalvsfix_linear_0.3}, ~\ref{fig:generalvsfix_nonlinear_0.5},~\ref{fig:generalvsfix_linear_0.0007},~\ref{fig:generalvsfix_nonlinear_0.0007} show that the testing performance of the model trained using a time-varying network is in fact almost as good as that trained for the fixed network setting. There is no benefit in training different LAA models for different fixed network settings.} For Figure~\ref{fig:generalvsfix_linear_0.3}, the testing was done for $q=0.3$ and a linear system. In Figure~\ref{fig:generalvsfix_nonlinear_0.5}, the chosen system is the nonlinear cartpole and $q=0.5$. Figure~\ref{fig:TimeVaryingNtwkTrain_0.007} shows the estimation error for very small values of $p$ and $q$. The LAA model trained over a time-varying network is seen to work well over a wide range of $p$ and $q$.

% \begin{figure}[h]
% 	\begin{center}
% 		\subfloat[]{\includegraphics[width = 0.5\linewidth]{Results/general_linear_0.3.pdf}
% 			\label{fig:generalvsfix_linear_0.3}}
% % % 		\subfloat[]{\includegraphics[width = 0.25\linewidth]{ICC-2021/Results/general_linear_0.5.pdf}
% % % 			\label{fig:generalvsfix_linear_0.5}}
% % 		\subfloat[]{\includegraphics[width = 0.25\linewidth]{ICC-2021/Results/general_nonlinear_0.3.pdf}
% % 			\label{fig:generalvsfix_nonlinear_0.3}}
% 		\subfloat[]{\includegraphics[width = 0.5\linewidth]{Results/general_nonlinear_0.5.pdf}
% 			\label{fig:generalvsfix_nonlinear_0.5}}
% 		\caption{\small Controls are communicated over the network. (a) Linear system $q=0.3$ (b) Nonlinear $q=0.5$. The corresponding results for $q=0.5$ and $q=0.3$ are similar.}	
%     	\label{fig:TimeVaryingNtwkTrain}		
% 	\end{center}
% 	\vspace{-0.125in}
% \end{figure}

\begin{figure}[t]
	\begin{center}
		\subfloat[]{\includegraphics[width = 0.5\linewidth]{Results/general_linear_0.3_barplot.pdf}
			\label{fig:generalvsfix_linear_0.3}}
% % 		\subfloat[]{\includegraphics[width = 0.25\linewidth]{ICC-2021/Results/general_linear_0.5.pdf}
% % 			\label{fig:generalvsfix_linear_0.5}}
% 		\subfloat[]{\includegraphics[width = 0.25\linewidth]{ICC-2021/Results/general_nonlinear_0.3.pdf}
% 			\label{fig:generalvsfix_nonlinear_0.3}}
		\subfloat[]{\includegraphics[width = 0.5\linewidth]
		{Results/general_nonlinear_0.5_nonlinear_barplot.pdf}
			\label{fig:generalvsfix_nonlinear_0.5}}
		\caption{\small Controls are communicated over the network. (a) Linear system $q=0.3$ (b) Nonlinear $q=0.5$. The corresponding results for $q=0.5$ and $q=0.3$ are similar.}	
    	\label{fig:TimeVaryingNtwkTrain}		
	\end{center}
	\vspace{-0.125in}
\end{figure}

\begin{figure}[t]
	\begin{center}
		\subfloat[]{\includegraphics[width = 0.5\linewidth]{Results/general_linear_0.0007.pdf}
			\label{fig:generalvsfix_linear_0.0007}}
% % 		\subfloat[]{\includegraphics[width = 0.25\linewidth]{ICC-2021/Results/general_linear_0.5.pdf}
% % 			\label{fig:generalvsfix_linear_0.5}}
% 		\subfloat[]{\includegraphics[width = 0.25\linewidth]{ICC-2021/Results/general_nonlinear_0.3.pdf}
% 			\label{fig:generalvsfix_nonlinear_0.3}}
		\subfloat[]{\includegraphics[width = 0.5\linewidth]
		{Results/general_nonlinear_0.0007.pdf}
			\label{fig:generalvsfix_nonlinear_0.0007}}
		\caption{\small Controls are communicated over the network for $q=0.007$. (a) Linear system (b) Nonlinear System.}	
    	\label{fig:TimeVaryingNtwkTrain_0.007}		
	\end{center}
	\vspace{-0.125in}
\end{figure}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \begin{table*}[t]
% \centering
% \begin{tabular}{@{}llllllll@{}}
% \toprule
% \textbf{} & \multicolumn{4}{c}{\textbf{Trained Model}} & \multicolumn{3}{c}{\textbf{Tested Over}} \\ \midrule
% \multicolumn{1}{|l|}{\textbf{$q$}} & \multicolumn{1}{l|}{\textbf{$p$}} & \multicolumn{1}{l|}{\textbf{Control}} & \multicolumn{1}{l|}{\textbf{System}} & \multicolumn{1}{l|}{\textbf{Compare}} & \multicolumn{1}{l|}{\textbf{No Age}} & \multicolumn{1}{l|}{\textbf{Age}} & \multicolumn{1}{l|}{\textbf{Noisy Age}} \\ \midrule
% \multicolumn{1}{|l|}{0.0007} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}$0.007$, $0.002$, $0.0034$, \\ $0.004$, $0.0068$, $0.00693$\end{tabular}} & \multicolumn{1}{l|}{\multirow{3}{*}{Known}} & \multicolumn{1}{l|}{\multirow{3}{*}{Linear}} & \multicolumn{1}{l|}{\multirow{3}{*}{TVKF}} & \multicolumn{1}{l|}{\multirow{3}{*}{}} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\ \cmidrule(r){1-2} \cmidrule(l){7-8} 
% \multicolumn{1}{|l|}{0.3} & \multicolumn{1}{l|}{$0.01$, $0.1$, $0.297$} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\ \cmidrule(r){1-2} \cmidrule(l){7-8} 
% 0.5 & \multicolumn{1}{l|}{$0.01$, $0.3$, $0.499$} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} &  &  \\ \bottomrule
% \end{tabular}
% \end{table*}
